HybridMIM: A Hybrid Masked Image Modeling Framework for 3D Medical Image Segmentation

Masked image modeling (MIM) with transformer backbones has recently been exploited as a powerful self-supervised pre-training technique. The existing MIM methods adopt the strategy to mask random patches of the image and reconstruct the missing pixels, which only considers semantic information at a lower level, and causes a long pre-training time.This paper presents HybridMIM, a novel hybrid self-supervised learning method based on masked image modeling for 3D medical image segmentation.Specifically, we design a two-level masking hierarchy to specify which and how patches in sub-volumes are masked, effectively providing the constraints of higher level semantic information. Then we learn the semantic information of medical images at three levels, including:1) partial region prediction to reconstruct key contents of the 3D image, which largely reduces the pre-training time burden (pixel-level); 2) patch-masking perception to learn the spatial relationship between the patches in each sub-volume (region-level).and 3) drop-out-based contrastive learning between samples within a mini-batch, which further improves the generalization ability of the framework (sample-level). The proposed framework is versatile to support both CNN and transformer as encoder backbones, and also enables to pre-train decoders for image segmentation. We conduct comprehensive experiments on four widely-used public medical image segmentation datasets, including BraTS2020, BTCV, MSD Liver, and MSD Spleen. The experimental results show the clear superiority of HybridMIM against competing supervised methods, masked pre-training approaches, and other self-supervised methods, in terms of quantitative metrics, timing performance and qualitative observations. The codes of HybridMIM are available at https://github.com/ge-xing/HybridMIM

==> tables/brats_ablation_old.tex <==
\begin{table}[t]
    \centering
    % 在BraTS2020数据集上进行消融实验。我们选择UNet与SwinTransformer作为backbone，逐个添加我们提出的不同层次的损失函数。其中LR为局部重建损失，Num为数量分布预测损失，Loc为位置分布预测损失，Consis为一致性损失，CL为对比学习损失。下游任务的分割结果展示了我们提出的每个损失函数对于不同架构的有效性。
    \caption{Ablation experiments are performed on the BraTS2020 dataset. We choose UNet and SwinTransformer as the backbone and add the different levels of loss functions we propose one by one. Where LR is the local reconstruction loss, Num is the number distribution prediction loss, Loc is the location distribution prediction loss, Consis is the consistency loss, CL is the contrastive learning loss. The segmentation results of the downstream task demonstrate the effectiveness of each of our proposed loss functions for different architectures.}
    % \vspace{-3mm}
    \label{tab:ablation}
    \renewcommand\arraystretch{1.0}
    \setlength\tabcolsep{5pt}%调列距
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c | c c c c c c c | c c c c c c}

    \hline
    \multirow{2}*{\makecell{Backbone}} & & \multicolumn{5}{c}{Loss} & &  & \multicolumn{4}{c}{Segmentation Target} & \\
    \cline{3-7} \cline{10-13}
     & & LR & Num & Loc & Consis & CL &&& WT & TC & ET & Avg & \\
    \hline
    \multirow{4}{*}{UNet} &  &  &  &  & & &&& 89.75 & 84.65 & 78.83 & 84.41 &\\
     & & \checkmark & & & & & & & 90.19 & 85.50 & 79.48 & 85.06 & \\
     & & \checkmark & \checkmark & & & & & & 90.05 & 85.48 & 79.97 & 85.17 & \\
     & & \checkmark & \checkmark & \checkmark & & & & & 90.15 & 85.65 & 80.10 & 85.30 & \\
     & & \checkmark & \checkmark & \checkmark & \checkmark & & & & 90.30 & 85.36 & {80.56} & 85.40 & \\
     & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & {90.62} & {86.28} & {80.17} & {85.69} & \\
     \hline
    \multirow{4}{*}{Swin} & & &  & & & & & & 90.08 & 85.19 & 80.01 & 85.09 & \\
     & & \checkmark & & & &  & & & 90.95 & 86.17 & 80.22 & 85.78 & \\
     & & \checkmark & \checkmark & & &  & & & 90.93 & 86.94 & 80.48 & 86.12 & \\
     & & \checkmark & \checkmark & \checkmark & &  & & & 91.18 & 86.33 & 81.10 & 86.20 & \\
     & & \checkmark & \checkmark & \checkmark & \checkmark &  & & & 90.98 & 87.06 & 80.71 & 86.24 & \\
     & & \checkmark & \checkmark &\checkmark & \checkmark & \checkmark & & & {91.48} & {86.88} & {80.81} & {86.39} & \\
    \hline
    \end{tabular}
    }
\end{table}



==> tables/dataset.tex <==
\begin{table*}[t]
    \centering
    % MP-SSL共使用4个不同器官的数据集进行实验，其中BraTS2020数据集为多模态数据，Spleen数据集只需要分割脾脏，其他数据集均为多目标分割数据集。剪裁大小为训练时输入的大小，PT-decoding size 为预训练时选择的局部重构区域大小。样本大小为数据集的规模。增强为训练时所用的数据增强方式。
    \caption{HybridMIM used a total of 4 datasets with different organs for the experiments. the BraTS2020 dataset is multimodal data, the Spleen dataset only needs to segment the spleen, and all other datasets are multi-target segmentation datasets. The crop size is the size of the input during training. Sample size is the size of the dataset. Augmentation is the data augmentation method used during training.}
    % \vspace{-3mm}
    \label{tab:data_intro}
    \renewcommand\arraystretch{1.3}
    \setlength\tabcolsep{10pt}%调列距
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c c c c c c | c}
    
    \hline
    Dataset & Modality & Object number & Crop size & Sample size & Augmentation \\
    \hline
    BraTS2020 & 4 & Brain tumor (3) & (128,128,128) & 369 & \multirow{4}{*}{\makecell{random flip \\ random rotate \\ random scale \\ random shift}} \\
    % \hline

    BTCV & 1 & Multi-organ (13) & (96,96,96)  & 30 &  \\
    % \hline

    Liver & 1 & Liver and tumor (2) & (96,96,96) &  201 &  \\
    % \hline

    Spleen & 1 & Spleen (1) & (96,96,96) & 61 &  \\
    \hline
    \end{tabular}
    }
% \vspace{-5mm}
\end{table*}


